GeomCA: Geometric Evaluation of Data Representations

Evaluating the quality of learned representations without relying on a downstream task remains one of the challenges in representation learning. In this work, we present Geometric Component Analysis (GeomCA) algorithm that evaluates representation spaces based on their geometric and topological properties. GeomCA can be applied to representations of any dimension, independently of the model that generated them. We demonstrate its applicability by analyzing representations obtained from a variety of scenarios, such as contrastive learning models, generative models and supervised learning models.

==> Sections/extras.tex <==
\begin{center}
\begin{tabular}{ |c||c|c|c| } 
 \hline
 & (a) & (b) & (c) \\
 \hline
 \hline
 $\eta_c, \eta_q$ & $0, 0$ & $0.3, 0.0$ & $0.3, 0.7$ \\ 
 \hline
 $P, R$ & $1.0, 1.0$ & $0.16, 0.16$ & $1.0, 0.64$ \\ 
 \hline
 $c(\mathcal{G}), q(\mathcal{G})$ & $1.0, 1.0$ & $1.0, 1.0$ & $0.78, 0.38$ \\ 
 \hline
 \hline
 $c(\mathcal{G}_0), q(\mathcal{G}_0)$ & $1.0, 0.49$ & $1.0, 0.25$ & $0.93, 0.43$\\
 \hline
 $c(\mathcal{G}_1), q(\mathcal{G}_1)$ & 
 $1.0, 0.43$ & $1.0, 0.5$ & $0.51, 0.75$ \\\hline
\end{tabular}
\end{center}

An example of geometric sparsification is shown in Figure \ref{fig:method:sparsification} with $\delta = x, y, z$. 

\begin{figure}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{Figures/sparsification.png}}
\caption{Example of sparsification procedure.}
\label{fig:method:sparsification}
\end{center}
\vskip -0.2in
\end{figure}




\begin{center}
\begin{tabular}{ |c|c|c||c| } 
 \hline
$|T|$, $|V|$ & $|T'|$ [time] & $|V'|$ [time] & $|\mathcal{G}|_\mathcal{V} + |\mathcal{G}|_\mathcal{E}$ [time]  \\
 \hline
 \hline
 $50000$ & $9380$ [1h 32min] & $5349$ [54min] & $18734$ [11min] \\ 
 \hline
 $10000$ & $2612$ [3min] & $1668$ [2min] & $5468$ [40s] \\ 
 \hline
 $5000$ & $1387$ [50s] & $888$ [31s] & $2930 [11s]$ \\ 
 \hline

 $1000$ & $390$ [2s] & $295$ [2s] & $863$ [1s]\\
 \hline
\end{tabular}
\label{tab:exp:stylegan_sparsification_time}
\end{center}





\begin{comment}
\begin{figure}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{Figures/boxes_examples.png}}
\caption{Examples of boxes.}
\label{fig:boxes-examples}
\end{center}
\vskip -0.2in
\end{figure}
\end{comment}

==> Sections/old_intuition.tex <==
\section{Method}

In this section, we introduce the proposed GeomCA algorithm. We present its intuitive idea in Section \ref{sec:method:idea} and its technical details in Section \ref{sec:method:alg}. % Lastly, we discuss connections to persistence homology in Section \ref{sec:method:ph}.

\subsection{Intuitive Idea} \label{sec:method:idea}
%The basic idea of the GeomCA algorithm is to analyze the topology and geometry of the space described by the given data representations. By topology we mean the global structure of the manifold $\mathcal{M}$ that these representations describe, while we use the term geometry to refer to the local properties of $\mathcal{M}$. In this work, we will focus on the global and local structure of the connected components of the manifold $\mathcal{M}$.

The basic idea of the GeomCA algorithm is to compare the global properties (topology) and local properties (geometry) of the {\color{blue} spaces} $R$ and $E$ representing the underlying true data manifold $\mathcal{M}$. We conclude that $E$ is a good representation of $\mathcal{M}$ if it is well aligned with the reference representation $R$. The aim is to be able to detect areas where $R$ and $E$ are coherent and quantify the degree of their alignment, as well as detect isolated individual representations (outliers) or groups of representations consisting of points from only one of the sets $R$ or $E$.

%The manifold $\mathcal{M}$ is in fact constructed from two discrete sets of representations, $R$ and $E$. By working with two sets rather than only one, 
% we can compare topological and geometric properties $\mathcal{M}$ with the ones of its restrictions $\mathcal{M}|_{T}$ and $\mathcal{M}|_{V}$ to the sets $R$ and $E$, respectively. [PROBLEMATIC] 

%we can analyse the global and local properties of $\mathcal{M}$ %with respect to 
%in terms of the points from these sets. More precisely, we analyse $\mathcal{M}$ by investigating how well the sets $R$ and $E$ align. Intuitively, $R$ and $E$ can be thought of as the ``training'' (or reference) set and the ``validation'' (or evaluation) set, respectively. The aim is to be able to detect areas in the representation space where $R$ and $E$ are coherent and quantify the degree of their alignment, as well as detect isolated individual representations (outliers) or groups of representations consisting of points from only one of the sets $R$ or $E$. %Therefore, we think of the set $R$ as the ``training'' (or reference) set, while $E$ represents the ``validation'' (or evaluation) set. 
In summary, we wish to answer the following two questions: 
\begin{enumerate}
    \item[(Q1)] %How many connected components of $\mathcal{M}_{T \cup V}$ there are and of what size? [Topology]
    Do $R$ and $E$ have the same number of connected components, and are their sizes comparable? [Topology]
    
    % Do the connected components of $\mathcal{M}_T$ differ from those of $\mathcal{M}_{T \cup V}$? [Topology]
     %change when additionally considering representations from $E$ (or $R$)? 
    \item[(Q2)] %How heterogeneous are the connected components of $\mathcal{M}_{T \cup V}$ in terms of points from $R$ and $E$? [Geometry]
    How much do the connected components of $R$ and $E$ overlap? [Geometry]
\end{enumerate}

%\begin{comment}
However, to be able to study any topological and geometric properties, and therefore answer the above questions, we must first obtain the manifoldanswering the above questions requires access to the manifold $\mathcal{M}_{T \cup V}$. Since the sets $R$ and $E$ are discrete, it is impossible to obtain $\mathcal{M}_{T \cup V}$ in an analytical form. One way to create volume from $T \cup V$ is by constructing a \textit{simplicial complex}. Since it is impossible to obtain $\mathcal{M}_{T \cup V}$ in an analytical form, we need to rely on an approximation that can be constructed from the discrete sets $R$ and $E$. 
One way to obtain such approximation is by constructing a \textit{simplicial complex}. Intuitively, a simiplicial complex, which is a standard construction in topology, enriches a set of points with edges, triangles and other high-order simplices if a certain distance condition is satisfied. An example of a simplicial complex used in this work is \textit{Vietoris-Rips complex} in which two points are connected by an edge if the distance between them is smaller than a given threshold. Similarly, three points are connected by a triangle if their pairwise distances are smaller than the given threshold (right panel). Following this procedure, higher-order simplices can be constructed. 


{\color{blue}
To answer these questions, we need to find the connected components of $R$ and $E$, compare their size, and quantify their alignment. For this, we build a ...  


}

\begin{figure}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{Figures/intuition_toy_example.png}}
\caption{An example of a Vietoris-Rips 1-skeleton with different radius parameters.}
\label{fig:method:vietoris-rips}
\end{center}
\vskip -0.1in
\end{figure}

In this work, we will work only with $1$-skeletons which contain only points and edges. Examples of such 1-skeletons of Vietoris-Rips complexes obtained using various distance thresholds are shown in Figure \ref{fig:method:vietoris-rips}, where we additionally marked points from $R$ and $E$ sets in blue and orange, respectively.  %In this work, we will work only with $1$-skeletons which contain only points and edges.
%In a Vietoris-Rips complex, two points are connected by an edge if the distance between them is smaller than a given threshold. 
In the left panel, where the distance threshold is low, points are exactly the components of the graph. Smaller components emerge in the middle panel, where we marked the added edges connecting points from $E$ with points from $R$ in gray. This mixed component grows even larger in the right panel, where additionally obtain two homogeneous components, one from $E$ and one from $R$.


Given a Vietoris-Rips complex, we can now answer questions (Q1) and (Q2). By studying the number connected components of the complex as well as their size we can immediately answer (Q1). For example, in the right panel of Figure \ref{fig:method:vietoris-rips} [... ADD IMAGE and TEXT], while all the examples in Figure \ref{fig:method:toy-data} have two connected components. In order to answer (Q2), we need to further analyse the local properties of each connected component of the complex. A straightforward estimation of the component heterogeneity is to simply count the number of points belonging to each of the sets $R$ and $E$. For example, in left panel of Figure \ref{fig:method:toy-data}, the Vietoris-Rips complex has two  heterogeneous connected components of different sizes. However, such estimation is unable to detect spurious components visualized in the middle panel of Figure \ref{fig:method:toy-data}. Here, points from both sets are not mixed but rather concatenated. We can mitigate this issue by additionally investigating the nature of the component edges: if the number of edges between points belonging to different sets is large, then the component is ``well mixed''. In Figure \ref{fig:method:toy-data}, such edges are colored with gray. In this way, we can quickly see that the outer component visualized in middle panel of Figure \ref{fig:method:toy-data} contains few gray edges and is therefore correctly detected as spurious. By jointly investigating the nature of the vertices and edges of a Vietoris-Rips graph, we also identify the outer component in the right panel as spurious as it contains less $E$ points out of which only half is well mixed with points from $R$. This intuitive idea is the main driver behind GeomCA, which we rigorously define in the following section.


%by studying the number connected components of the complex \textit{and} their consistency in terms of points from the sets $R$ and $E$, respectively. The latter is of crucial importance for assessing the representations and explains the need for generating two sets of representations. We elaborate this fact on the following example: assume we chose two sets of representations that have semantically similar content. To check if the learned representations are coherent, we perform the above analysis on the components of the Vietoris-Rips complex they describe. If the components have equal amount of points from both sets as well as good connectivity between the points of different sets (discussed below), we can conclude that the representations are consistent. Examples of both coherent and non coherent sets of representations are shown in Figure \ref{fig:method:toy-data} in the left columns.

%The information about the consistency of connected components in terms of the two sets of points can obtained from their geometry and is two-folded. As briefly mentioned above, we can not only study the number of points from both sets contained in a component but also their connectivity. The latter is in fact important for detecting spurious components such as the one visualised in Figure \ref{fig:method:toy-data}. Here, points from both sets are not mixed but rather concatenated, but nonetheless form one connected component due to their distance. This issue can be mitigated by investigating the nature of the edges: if the number of edges between points belonging to different sets is large, the component is of high-quality (see Figure) otherwise it is of low quality as shown in Figure. We rigorously define this idea in the following section.


\begin{figure*}[ht]
\vskip 0.2in
\centering
\begin{center}
\centerline{\includegraphics[width=0.9\textwidth]{Figures/toy_components.png}}
\caption{2-dimensional examples of sparsified data points and the corresponding GeomCA visualization.}
\label{fig:method:toy-data}
\end{center}
\vskip -0.2in
\end{figure*}

\subsection{GeomCA Algorithm} \label{sec:method:alg}
Let $X = \{ x_i \}_{i = 1}^{n_X} \subset \mathbb{R}^M$ be the dataset of observations and let $Z = \{ z_i \}_{i = 1}^{n_X} \subset \mathbb{R}^N$ denote the corresponding representations obtained from any model $\mathbb{M}$, i.e., $Z = \mathbb{M}(X)$. In a typical machine learning setup, we additionally assume that $N \ll M$, although this assumption is not necessary for GeomCA to work. Let $R = \{ z_i \}_{i = 1}^{n_R} \subset Z$ and $E = \{ z_i \}_{i = 1}^{n_E} \subset Z$ be two subsets of the set of representations for which we assume that $n_R + n_E \le n_X$ and $R \neq E$. The latter assumption is needed in order to obtain meaningful insights as it eliminates the case where $R$ and $E$ are perfectly aligned. While GeomCA provides most insight into representations when $R \cap E = \emptyset$, a non-empty intersection $\emptyset \neq R \cap E \subsetneq R \cup E$ might desirable in situations where it is important to investigate deviations from the intersection $R \cap E$ [IS THIS SUFFICIENT?]. 

Our algorithm, summarized in Algorithm \ref{alg:geomCA-alg}, consists of two phases: \textit{manifold approximation} and \textit{manifold evaluation} phases. The former extracts topological (global) information from the set of representations $R \cup E$ by approximating the manifold $\mathcal{M}$ and extracting its connected components. From each of the obtained connected components, we then extract geometric (local) information in the latter phase. We describe each of these phases in detail in the rest of the section.
[CONNECT THIS SECTION WITH FIGURE EXAMPLE]

\noindent \textbf{Manifold approximation} Our first goal is to obtain an approximation of the manifold $\mathcal{M}_{R \cup E}$ from the union of points $R \cup E$. As intuitively explained in Section \ref{sec:method:idea}, we achieve this by constructing a Vietoris-Rips simplicial complex. Since constructing higher-order simplices is computationally expensive, we simplify this construction by considering 1-skeletons of simplicial complexes containing only points and edges between them. Therefore, these form a Vietoris-Rips graph defined below.

\begin{definition} \label{def:vr}
A Vietoris-Rips graph on the set of points $W$ with respect to a radius $\varepsilon > 0$ is a graph $\mathcal{G}_\varepsilon(W) = (\mathcal{V}, \mathcal{E})$ with vertices $\mathcal{V} = W$ and edges $\mathcal{E} = \{ e_{ij} = (v_i, v_j) \subset \mathcal{V} \times \mathcal{V} \, | \, d(v_i, v_j) < \varepsilon \}$.
\end{definition}

We built a Vietoris-Rips graph $\mathcal{G} := \mathcal{G}_\varepsilon(R \cup E)$ on the union $R \cup E$. We discuss the choice of the radius $\varepsilon$ in Section \ref{sec:epsilon_selection}. For clarity of the remainder of the section, we introduce the following notation. Firstly, we denote by $\mathcal{G} := \sqcup_i \mathcal{G}_{i}$ the graph-connected components of $\mathcal{G}$. By a restriction of a graph $\mathcal{G}$ to a subset of $W$, we mean the subgraph $\mathcal{G}^W$ of $\mathcal{G}$ with vertex and edge sets restricted to $W$. For example, a connected component $\mathcal{G}_i$ restricted to the set $R$ is a graph $\mathcal{G}_i^R$ obtained by removing all the points $E$ as well as all the edges from and to them from the vertex and edge sets of $\mathcal{G}_i$. Lastly, we denote by $|\mathcal{H}|_\mathcal{V}$ and $|\mathcal{H}|_\mathcal{E}$ the cardinalities of the vertex set and edge set of any given graph $\mathcal{H}$, respectively.

\noindent \textbf{Manifold evaluation} The goal of this phase is to analyze the connected components of the manifold $\mathcal{M}_{R \cup E}$ approximated with the Vietoris-Rips graph $\mathcal{G}$ constructed in the previous phase. As mentioned in Section \ref{sec:method:idea}, we study the geometrical properties of its connected components, $\mathcal{G}_i$, with respect to representations from the sets $R$ and $E$.  In particular, we study (a) their heterogeneity determined by the ratio of representations from $R$ and $E$ contained in it, and (b) the heterogeneity of edges among them determining the quality. We refer to these geometric properties as \textit{consistency} and \textit{quality} of connected components, respectively, and rigorously define them in the following.

\begin{definition} \label{def:comp-consistency}
Consistency $c$ of a component $\mathcal{G}_i$ is defined as the ratio 
\begin{equation}
    c(\mathcal{G}_i) = 1 - \frac{|\, |\mathcal{G}_i^R|_\mathcal{V} - |\mathcal{G}_i^{E}|_\mathcal{V} \,|}{|\mathcal{G}_i|_\mathcal{V}}.
\end{equation}
\end{definition}

A component $\mathcal{G}_i$ will attain high consistency score $c(\mathcal{G}_i)$ if it contains equally many representations from $R$ and $E$. We call such component \textit{heterogeneous} or \textit{diverse}. On contrary, $c(\mathcal{G}_i)$ will be low if $\mathcal{G}_i$ is dominated by points from only one of the sets $R$ ad $E$, in which case $\mathcal{G}_i$ is said to be \textit{homogeneous}. Examples of both heterogeneous and homogeneous components are shown in Figure \ref{fig:method:toy-data}.  However, as seen in the middle panel, consistency itself is not a sufficient measure for evaluating components. In this case, a component is diverse in terms of vertices but not in terms of edges as the number of edges among representations from $R$ and $E$ is low. This is measured by component quality, defined below.

\begin{definition} \label{def:comp-quality}
Quality of a component $\mathcal{G}_i$ is defined as the ratio
\begin{equation}
    q(\mathcal{G}_i) = \frac{|\mathcal{G}_i|_\mathcal{E} - | \mathcal{G}_i^{R}|_\mathcal{E} + |\mathcal{G}_i^{E}|_\mathcal{E}}{|\mathcal{G}_i|_\mathcal{E}}. 
\end{equation}
\end{definition}

Similarly as for the consistency score, a component $\mathcal{G}_i$ will attain high quality score, if it exhibits good connectivity among representations from $R$ and $E$ it contains. Such component is said to be of \textit{high quality} and have \textit{heterogeneous edges}. On the other hand, if edges in $\mathcal{G}_i$ exist only among points from one of the sets $R$ or $E$, the component achieves low quality score and is said to be of \textit{low quality} and its edges \textit{homogeneous}. 

The consistency and quality measures can however be also used in several ways to obtain a global score over the entire Vietoris-Rips graph. Firstly, we simply generalize Definitions \ref{def:comp-consistency} and \ref{def:comp-quality} to $\mathcal{G}$. 

\begin{definition}
We define $c(\mathcal{G})$ as \textit{network consistency}, and $q(\mathcal{G})$ as \textit{network quality}. 
\end{definition}

The global network consistency and quality are important measures to detect imbalances between the sets $R$ and $E$. This is especially applicable in large-scale experiments where the sizes of $R$ and $E$ are reduced for computational purposes. We discuss such reduction in Section \ref{sec:gamma} and demonstrate the usefulness of network consistency and quality measures in such situations in Section \ref{sec:exp:gan}. 

Next, we aggregate the components of certain consistency and quality into two more global scores, precision and recall.

\begin{definition} \label{def:geom-pr}
Let $\eta_c, \eta_q \in [0, 1]$ be real numbers. Let
\begin{equation}
    \mathcal{S}(\eta_c, \eta_q) = 
    \bigcup_{\substack{ q(\mathcal{G}_i) > \eta_q, \\ c(\mathcal{G}_i) > \eta_c}} \mathcal{G}_i
\end{equation}
be the union of the connected components $\mathcal{G}_i$ with the minimum consistency and quality score determined by $\eta_c$ and $\eta_q$, respectively. Let $\mathcal{S}(\eta_c, \eta_q)^R$ and $\mathcal{S}(\eta_c, \eta_q)^E$ denote the restrictions of $\mathcal{S}(\eta_c, \eta_q)$ to the sets $R$ and $E$, respectively. We define precision $\mathcal{P}$ and recall $\mathcal{R}$
with respect to the thresholds $\eta_c, \eta_q$ as 
\begin{equation}
    \mathcal{P} = \frac{|\mathcal{S}^E|_\mathcal{V}}{|\mathcal{G}^E|_\mathcal{V}} \quad \mathcal{R} = \frac{|\mathcal{S}^R|_\mathcal{V}}{|\mathcal{G}^R|_\mathcal{V}},%\quad N = \frac{|\mathcal{S}^T|_\mathcal{V} + |\mathcal{S}^V|_\mathcal{V}}{|\mathcal{G}|_\mathcal{V}}
\end{equation}
respectively, where we omitted the explicit dependency on $\eta_c, \eta_q$ for simplicity. 
\end{definition}

The thresholds $\eta_c$ and $\eta_q$ determine the level of alignment between sets $R$ and $E$ that we wish to consider. A high value of $\eta_c$ requires the components to be equally well represented by the sets $R$ and $E$, while a high value of $\eta_q$ additionally requires that the points from $R$ and $E$ in each component are well mixed and consistent. The effect of these thresholds in investigated in Section \ref{sec:exp:multiview-box}. 


\input{Sections/algorithm}


\subsection{Implementation details} \label{sec:implementation-details}
In this section, we provide additional implementation details that were deployed in order to speed up and automate the algorithm.  

\subsection{Selecting Vietoris-Rips radius $\varepsilon$} \label{sec:epsilon_selection}
The structure of Vietoirs-Rips graph $\mathcal{G}$ depends on the hyperparameter $\varepsilon$ determining the maximum length of its edges. Extracting the true underlying value of $\varepsilon$ is a non-trivial task, especially in higher dimensional representation space. For $\varepsilon$ too small, each point will be contained in its own component, while $\varepsilon$ too large will connect all the points into one single component. The true $\varepsilon$ that results in the approximation of $\mathcal{M}$ that reflects the correct topology of the space, lies between these two extreme choices. A more precise estimate could be determined by topological algorithms, such as persistent homology CITE. However, due to computational and scalability issues of this approach, we instead either choose a specific value of $\varepsilon$ or estimate it empirically by examining the distances in the reference set $R$. We randomly sample $2k$ of representations from $R$ and calculate their pairwise distances $D = \{ d(z_i, z_j) | \, i=1, \dots k \\ j = k, \dots, 2k \}$. We then set $\varepsilon$ as $p$th percentile of the set $D$ and denote it by $\varepsilon = \varepsilon(p)$.

\subsection{Reducing the number of representations} \label{sec:gamma}
As seen from Definition \ref{def:vr}, the construction of the Vietoris-Rips graph involves calculation of pairwise distances among points in $R \cup E$. Such calculation can become a computational burden when analyzing large sets of representations. One way to reduce the number of representations in the sets $R$ and $E$ without loosing the topological information is to perform \textit{geometric sparsification} defined below.

\begin{definition}
A geometric sparsification of a set $W$ with respect to a sparsificaltion distance $\delta > 0$ is a subset $W' \subset W$ such that $d(w_i, w_j) > \delta$ for every $w_i, w_j \in W'$, $i \neq j$.
\end{definition}

The sparsificaiton parameter $\delta$ determines the severity of data reduction, where larger $\delta$ results in sparser point cloud. We perform geometric sparsification on the sets $R$ and $E$ separately, such that we can construct the Vietoris-Rips graph more efficiently using the obtained sparse sets $R'$ and $E'$. The reason for separate sparsification of $R$ and $E$ is to be able to detect potential differences in their topology. Intuitively, if $R$ and $E$ reflect the structure of the same representation space, then so should the sparsified sets.
%keep the distinction among the two sets which is lost if sparsification is performed on $T \cup V$. 

The choice of $\delta$ is closely connected to the choice of the Vietoris-Rips radius $\varepsilon$. As $\delta > \varepsilon$ would generate only isolated components, $\delta$ should be chosen from the interval $[0, \varepsilon]$. Intuitively, if $\delta = \epsilon$, a component in Vietoris-Rips graph $\mathcal{G}$ is created only when points from $R$ and $E$ are well mixed. This means that between every pair of points from one set (e.g., $R$) there necessarily needs to exists a point from the other set (e.g., $E$) that is less than $\epsilon$ apart from both of the points from the first set (e.g., $R$). On the other hand, if $\delta < \varepsilon$, we still allow points from each of the set to get connected without having a ``witness'' from the other set. Regardless of the choice of $\delta$, the sparsification process will keep the subset of the most outer points. [IS THIS A RISKY STATEMENT?]. 


